In-Vivo Bytecode Instrumentation for Improving Privacy on Android Smartphones in Uncertain Environments

In this paper we claim that an efficient and readily applicable means to improve privacy of Android applications is: 1) to perform runtime monitoring by instrumenting the application bytecode and 2) in-vivo, i.e. directly on the smartphone. We present a tool chain to do this and present experimental results showing that this tool chain can run on smartphones in a reasonable amount of time and with a realistic effort. Our findings also identify challenges to be addressed before running powerful runtime monitoring and instrumentations directly on smartphones. We implemented two use-cases leveraging the tool chain: BetterPermissions, a fine-grained user centric permission policy system and AdRemover an advertisement remover. Both prototypes improve the privacy of Android systems thanks to in-vivo bytecode instrumentation.

==> figures/android-stack.tex <==
%% Android Software Stack

\tikzset{
>=stealth',
  punktchain/.style={
    rectangle, 
    rounded corners, 
    draw=black, very thick,
    text width=10em, 
    text centered, 
    on chain},
  line/.style={draw, thick, <-},
  element/.style={
    tape,
    top color=white,
    bottom color=blue!50!black!60!,
    minimum width=8em,
    draw=blue!40!black!90, very thick,
    text width=10em, 
    text centered, 
    on chain},
  every join/.style={->, thick,shorten >=1pt},
  decoration={brace},
  tuborg/.style={decorate},
  tubnode/.style={midway, right=2pt},
}
\tikzstyle{block} = [draw,fill=white!20,minimum width=4em]
\begin{tikzpicture}
  [node distance=.1cm,
  start chain=going below,]
     \node[punktchain] (applications) {Applications};
				\begin{scope}[start branch=hoejre,]
      		\node (applicationsPl) [block, on chain=going right] {Java};
    		\end{scope}
     \node[punktchain] (framework)      {Framework};
				\begin{scope}[start branch=hoejre,]
      		\node (frameworkPl) [block, on chain=going right] {Java/C/C++};
    		\end{scope}
     \node[punktchain] (libraries)      {Libraries + Dalvik VM};
				\begin{scope}[start branch=hoejre,]
      		\node (librariesPl) [block, on chain=going right] {C/C++};
    		\end{scope}
     \node[punktchain] (kernel) {Kernel};
				\begin{scope}[start branch=hoejre,]
      		\node (kernelPl) [block, on chain=going right] {C};
    		\end{scope}

			\draw[black] let
			    \p1=(kernel.west), \p2=(kernel.east) in
					    ($(\x1-4em,\y1+0.9em)$) -- ($(\x2+4em,\y2+0.9em)$) node[above, midway]  {};
			\draw[tuborg, decoration={brace}] let
			    \p1=(kernel.south), \p2=(kernel.north) in
					    ($(-2,\y1)$) -- ($(-2,\y2)$) node[tubnode, on chain=going left]  {Kernel mode};
			\draw[tuborg, decoration={brace}] let
			    \p1=(libraries.south), \p2=(applications.north) in
					    ($(-2,\y1)$) -- ($(-2,\y2)$) node[tubnode, on chain=going left]  {User mode};

  \end{tikzpicture}


==> figures/heapSizeHistogram-jimple.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5668.00,3968.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1210,1029){\makebox(0,0)[r]{\strut{} 100}}%
      \put(1210,1355){\makebox(0,0)[r]{\strut{} 200}}%
      \put(1210,1680){\makebox(0,0)[r]{\strut{} 300}}%
      \put(1210,2006){\makebox(0,0)[r]{\strut{} 400}}%
      \put(1210,2331){\makebox(0,0)[r]{\strut{} 500}}%
      \put(1210,2657){\makebox(0,0)[r]{\strut{} 600}}%
      \put(1210,2982){\makebox(0,0)[r]{\strut{} 700}}%
      \put(1210,3308){\makebox(0,0)[r]{\strut{} 800}}%
      \put(1342,484){\makebox(0,0){\strut{} 5}}%
      \put(1786,484){\makebox(0,0){\strut{} 10}}%
      \put(2230,484){\makebox(0,0){\strut{} 15}}%
      \put(2674,484){\makebox(0,0){\strut{} 20}}%
      \put(3118,484){\makebox(0,0){\strut{} 25}}%
      \put(3562,484){\makebox(0,0){\strut{} 30}}%
      \put(4006,484){\makebox(0,0){\strut{} 35}}%
      \put(4450,484){\makebox(0,0){\strut{} 40}}%
      \put(4894,484){\makebox(0,0){\strut{} 45}}%
      \put(5338,484){\makebox(0,0){\strut{} 50}}%
      \put(440,2006){\rotatebox{90}{\makebox(0,0){\strut{}Correctly Processed Applications}}}%
      \put(3340,154){\makebox(0,0){\strut{}Java Heap Size (MiB)}}%
      \put(3340,3638){\makebox(0,0){\strut{}Heap Size Influence on the Number of Correctly Processed Applications}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./figures/heapSizeHistogram-jimple.eps_tex}}%
    \gplfronttext
  \end{picture}%
\endgroup

